Transforming EU Governance: The Digital Integration through EBSI and GLASS

Traditionally, government systems managed citizen identities through disconnected data systems, using simple identifiers and paper-based processes, limiting digital trust and requiring citizens to request identity verification documents. The digital era offers a shift towards unique digital identifiers for each citizen, enabling a 'citizen wallet' for easier access to personal documents like academic records and licences, with enhanced security through digital signatures. The European Commission's initiative for a digital wallet for every EU citizen aims to improve mobility and integration, leveraging the European Blockchain Services Infrastructure (EBSI) for harmonised citizen integration. This paper discusses how EBSI and the GLASS project can advance governance and streamline access to identity documents.

==> 01_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Executive Summary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Introduction}
In recent years there has been an increased demand from citizens, corporations, and governments to access e-government services. This requires the need for trustworthy e-governance solutions that provide citizens and businesses with safe and transparent public services, and without compromising their security or privacy. The failure to satisfy these necessities can have severe economic and social consequences. Along with security and privacy, creating an infrastructure that users can rely on is a key consideration when establishing e-government \cite{leiding2021machine}, along with providing a strong linkage between digital identity and socio-economic inclusion \cite{addo2021advancing}.

Coursey \emph{et al.} predict that \emph{e-government will fundamentally transform the relationship between governments and citizens}  \cite{coursey2008models}. This transformation could lead to improved democracy, including around citizen participation, increased transparency, improved trust in government, strengthened democracy, and social inclusion \cite{draheim2020narratives}. But approaches to e-governance can fail without a citizen focus, increased accountability, citizen empowerment, co-production and good governance \cite{draheim2020narratives}. But, Draheim et al  \cite{draheim2020narratives} also outline that there are important political topics which must run alongside any development of e-governance applications including those related to the digital divide, anti-corruption, the loss of privacy, social change, and increasing control from government agencies. 

Valdavida \emph{et al.} \cite{valdavida2021public} outline a number of key recommendations in building a trustworthy approach to e-governance, including:

\begin{itemize}
\item \textbf{Bridge with the existing world.} This should allow for seamless integration with existing systems, and break-down the barriers to the exchange of digital assets from heterogeneous systems \cite{valdavida2021public}. 
\item \textbf{Law and technology.} This requires that legal and technology specialists work together to develop an integrated system. 
\item \textbf{Decentralisation, transparency and accountability.} This moves award from our requirements for centralised services, and aims to increase transparency, privacy and accountability \cite{valdavida2021public}.
\item \textbf{Value proposition.} This requires a strong focus on useful use cases which are important in the lives of citizens.
\item \textbf{Governance.} This should provide a well-defined foundation for the system based on roles, responsibilities, and decision-making processes and where the governance structures are well-defined, and clearly articulated at every stage of the development \cite{valdavida2021public}.
\end{itemize}


GLASS \footnote{\label{myfootnote}GLASS is funded within the EU Horizon 2020 research and innovation programme under grant agreement 959879} \cite{lo2022glass} provides a user-centric approach in which digital credentials are referenced within digital wallets owned and controlled by individuals. This eliminates the need for a third party to maintain trust. Citizens then have complete control over their identities and associated data. GLASS employs a trusted framework to enable the requester (often defined as the \emph{relying party}) to validate the verifiability of the issuer's verifiable credentials and digital signature. In the EU, these transfers must be compliant with the General Data Protection Regulation (GDPR) \cite{voigt2017eu} and the incorporation of a legal framework for electronic Identification and Authentication and trust Services (eIDAS). As a result, the GLASS model is able to carry out procedures that are functional across borders and in a user-friendly manner, in order to support  governments, citizens, organisations, and public services. The EBSI infrastructure provides a foundation element of this, and which can be used to provide trusted identity-checking services for citizens and trusted organisations. This infrastructure can provide a distributed infrastructure that can reduce administrative burdens and thus connect public administrations across all the EU state members. 

In this paper, we investigate EBSI and GLASS and examine their approaches to handling identity, security and privacy. In addition, we investigate the viable integration of GLASS and EBSI models. Overall, it focuses on a distributed, secure, and scalable e-Government architecture that integrates the GLASS \cite{glass_definition, GLASS-home} and EBSI (European Blockchain Services Infrastructure) projects \cite{EBSI-ec-dbb-wiki-home}. Both of these projects use permissioned blockchains and distributed ledger methods, in order to ensure security and privacy and can address some of the weaknesses of current e-government systems and the interoperability between governance departments. In order to provide improved resilience, GLASS has the option to use IPFS (InterPlanetary File System).

The rest of the paper is structured as follows. Section \ref{related_work} briefly describes the related work while Section \ref{data_sharing} presents fundamental data-sharing use cases. Section \ref{ipfs_usecases} proceeds with the presentation of IPFS use cases while Section \ref{eu_eid} summarises the European approaches for electronic identities. Soon afterwards Section \ref{eu_blockchain_part} details the European Blockchain Partnership while Section \ref{sec:Background} provides the necessary background information for the GLASS project. This enables Section \ref{glass_ebsi} to explain the feasibility of bringing together GLASS with EBSI. Last, Section \ref{sec:Conclusion and future work} draws the conclusions while giving some pointers for future work.











==> 02_related_work.tex <==
%% Completely restructure all of the related work
\section{Related work}
\label{related_work}

Lykidis \emph{et al.} \cite{lykidis2021use} define a wide range of ongoing blockchain-based e-Government applications including for authentication, e-Voting, land property services, e-Delivery Services, human resources management, and government contracting. Most of these integrate some form of identity management, but the approaches taken for identity management vary widely. Rathee and Singh \cite{RATHEE2021} thus provide a literature review of blockchain-related identity management. The two main approaches to identity management can be summarised as: 
\begin{itemize}
\item{using one or more appointed trusted authorities providing assurance over the identity-proofing of subjects,}
\item{allowing subjects to create and manage self-asserted identities, referred to as self-sovereign identities (SSI).}
\end{itemize}




\subsection{Country-wide adoption}
SSI is increasingly employed in blockchain-based applications, diverging from the traditional reliance on appointed trusted authorities evident in Public Key Infrastructure (PKI). Various projects, such as China's Blockchain Service Network (BSN) \cite{tang2022blockchain}, exemplify this shift. Similarly, Telechain in India, as defined by Singanamalla \emph{et al.} \cite{singanamalla2022telechain}, collaborates with telecommunication providers to meet regulatory requirements. Estonia's X-Road system, incorporating the Guardtime blockchain solution \cite{buldas2013keyless}, integrates state registries \cite{draheim2020blockchains}. Belarus's cryptohub HTP \cite{bazhenova2018digitalization} signifies its digital economy advancement, defining cryptographic operators and cryptocurrency exchanges. Akpan \emph{et al.} \cite{akpan2022governance} found a significant correlation between e-governance and governance in West Africa, emphasising the integration with established institutions.

In the EU, blockchain is increasingly considered for e-governance, yet challenges remain in aligning identity linkages with PKI and Qualified Digital Certificates. Turkanovic et al. \cite{turkanovic2020signing} suggest an architecture using CEF components like EBSI, eSignature, and eID compliant with eIDAS.


\subsection{Self-sovereign identity}
SSI enables individuals to create and control their identities using a key pair; transactions are signed digitally with a private key and verified with a public key, the former being securely stored in a citizen wallet inaccessible to others.

Globally, initiatives like The Open Identity Exchange (OIX) and Trust over IP Foundation (ToIP) \cite{ToIP} strive to standardise verifiable credentials and wallets. ToIP emphasises decentralised digital identity, issuing guidelines for Hyperledger Aries, Indy, and verifiable credentials \cite{Dizme2020}. The SSI framework encompasses the user (holder), credential issuer, and relying party, with the user managing credential acquisition and transfer. Trust is established via the issuer's digital signature and verification against their trusted public key.

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/toip.png}
%\captionsetup{justification=centering}
%\caption{Open Identity Exchange and Trust over IP \cite{ToIP}}
%\label{fig:openid}
%\end{center}
%\end{figure}

% Figure \ref{fig:toip2} illustrates the flexibility of the SSI approach. 

% In the scenario that follows, it is assumed that a user already created a digital ID, which contains various credentials.  We refer to these credentials as foundational credentials. These can be self-issued or third-party issued. Depending on the issuer and the type of credential, these credentials contain different attributes and have different legal effects. When a user subsequently wants to open a bank account, a redirection takes place to the user's digital ID. The user selects an issuer that is capable of creating a credential that satisfies the bank's rules and provides a relevant credential. The issuer verifies this, and upon successful verification, issues an identity proof of the user to the bank that provides identity-related evidence to support the account opening. 


%\begin{figure}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/toip2.png}
%\captionsetup{justification=centering}
%\caption{Open Identity Exchange and Trust over IP \cite{ToIP}}
%\label{fig:toip2}
%\end{center}
%\end{figure}

\subsection{Appointed trusted authorities}
Appointed trusted authorities in digital applications ensure identity-proofing for natural persons through centralised or decentralised registers and business registers for legal entities. Anand and Brass \cite{AnandNishant2021Rifd} examine eID systems and their governance.

\subsection{Sharing credentials}
Liang \emph{et al.} \cite{liang2017integrating} applied Hyperledger Fabric for consent-based healthcare data sharing with insurers. Data transactions are recorded on the blockchain, ensuring accountability. The system uses Hyperledger Fabric's membership service and channel scheme, featuring:

\begin{itemize}
\item \textbf{Membership service provider (CA)} for enrollment, certificate issuance, and access control during channel setup.
\item \textbf{Chaincode} for transaction management and participant isolation.
\end{itemize}

The License accoUntability and CompliancE (LUCE) platform on Ethereum \cite{havelange2019luce} aligns with GDPR, allowing data rectification and erasure. It involves Data Providers, Requesters, and Supervisory Authorities, covering:

\begin{itemize}
\item Document sharing, data access, compliance monitoring, and GDPR rights enforcement.
\end{itemize}

Jaiman \emph{et al.} \cite{jaiman2020consent} designed a blockchain-based health data consent model, incorporating smart contracts and Ethereum blockchain ontologies:

\begin{itemize}
\item Data Use Ontology (DUO) for consent.
\item Automatable Discovery and Access Matrix (ADA-M) for data request formatting.
\end{itemize}

\subsection{Right to be forgotten}\label{sect:5.1}
Centralised data storage can shift to distributed models like IPFS, which uses content hashing for file distribution. However, IPFS struggles with content deletion and limited encryption. Politou \emph{et al.} \cite{politou2020delegated} discuss GDPR's Right to be Forgotten (RtbF), highlighting the challenges in IPFS content erasure. They suggest an anonymous protocol for delegated erasure requests restricted to original content providers or their delegates.

%\begin{figure*}
%\centering
%\includegraphics[width=0.8\linewidth]{figures/erase.png}
%\caption{Erasure in IPFS %\cite{politou2020delegated}}
%\label{erase}
%\end{figure*}

\subsection{Dual-chain approaches}
Wang \emph{et al.} \cite{wang2018data} propose a dual blockchain approach for data sharing, with one chain storing original data and another for transaction records. This method segments data into $n$ blocks and allows transaction traceability. Data owners sign a random hash of a prior transaction, specifying the data block number, permission level, and the following user's public key. Access levels are categorised as:

\begin{itemize}
\item Level 1: Full rights to use and distribute data.
\item Level 2: Rights to use data and grant usage rights.
\item Level 3: Basic data usage rights.
\end{itemize}

\subsection{File sharing}
Khatal \emph{et al.} \cite{khatal2021fileshare} introduced FileShare, a secure, decentralised Ethereum-based file-sharing application. It registers users and ensures file provenance and traceability through smart contracts, managing encrypted file versions.

\section{Data sharing use cases}
\label{data_sharing}
Exploring data sharing and citizen integration in various application areas is crucial for developing distributed e-governance applications.

\subsection{Healthcare sharing}
Electronic Health Records (EHR) containing sensitive data require secure, efficient sharing among healthcare entities and patients, with strong encryption and consent protocols \cite{dubovitskaya2017secure,papadopoulos2021privacy}. Siyal \emph{et al.} \cite{siyal2019applications} identify blockchain's potential in healthcare for transparency, security, and cost efficiency but also note challenges in interoperability and standardisation.

Omran \emph{et al.} \cite{omran2022sharded} developed a sharded, privacy-enhanced blockchain for sharing pandemic-related diagnostic tests, using ring signatures for anonymity. They demonstrated significant efficiency improvements in data sharing for healthcare research.

\subsubsection{MedChain}
MedChain, implemented by Shen \emph{et al.} \cite{shen2019medchain}, exemplifies information sharing in healthcare, focusing on citizen permissions and interoperability. Its architecture employs a super-peer model at the highest level.

\subsubsection{Tangle-based}
Zheng \emph{et al.} \cite{zheng2019accelerating} designed a health data-sharing system using the IOTA Tangle with Masked Authenticated Messaging. IOTA users create and subscribe to channels for data publication and reception. IOTA integrates with EBSI in several domains, including credential management, SME financing, and data sharing \cite{IOTAEBSI}.

\subsection{Distributed Data Sharing Platforms}
\subsubsection{Distributed Health Care} 
Theodouli \emph{et al.} \cite{theodouli2018design} outlined a blockchain-based, layered healthcare architecture. Layer 1 involves Web/Cloud Platforms; Layer 2, Cloud Middleware; and Layer 3, the Blockchain Network. The system uses smart contracts with a Registry Contract (RC) for each patient's user registry and Patient Data Contracts (PDC), storing hashed data and URLs for healthcare data access. A Permissions Contract (PC) links PDCs with requesting entities and patient approvals.


%\begin{figure*}
%\centering
%\includegraphics[width=0.8\linewidth]{figures/baas.png}

%\caption{System architecture %\cite{theodouli2018design}}
%\label{Theodouli}
%\end{figure*}

%\begin{figure*}
%\centering
%\includegraphics[width=0.6\linewidth]{figures/baas2.png}

%\caption{Smart contract structure  %\cite{theodouli2018design}}
%\label{Theodouli2}
%\end{figure*}


Several approaches are being explored in managing EHR using blockchain technology \cite{holbl2018systematic}. Yüksel \emph{et al.} \cite{yuksel2017research} discuss EHR storage in distributed and cloud designs, proposing a centralised model by adapting decentralised Cloud architecture techniques. This cloud architecture involves structured storage of medical records with remote service providers, ensuring scalability, availability, and cost-effectiveness through security measures like identity management and policy integration \cite{abbas2014review}.

MedRec, a permissionless blockchain application on Ethereum \cite{azaria2016medrec}, demonstrates decentralised EHR management with auditable features. However, it raises concerns about transaction scalability and potential linkability, risking data and user anonymity. This has led to further research to address these issues \cite{yang2017blockchain}.

MediBchain \cite{al2017medibchain}, a permissioned, Ethereum-based peer-to-peer system, employs a cloud server for scalability. Despite encrypted data storage, linkability and unmeasurable transaction costs still need to be addressed. Bocek \emph{et al.} \cite{bocek2017blockchains} introduced an IoT (Internet of Things) based Ethereum architecture in Modum.io for the pharmaceutical supply chain. While promising, its partial decentralisation and vulnerability to HTTP server attacks make it unsuitable for sensitive EHR data.

\subsubsection{Permissioned approaches}
Stamatellis \emph{et al.} \cite{stamatellis2020privacy} used Hyperledger Fabric to create a privacy-preserving healthcare scenario, employing private data collection and Idemix suite for enhanced privacy and anonymity. Idemix, a Zero-Knowledge Proof protocol, ensures credential anonymity and unlinkability \cite{stamatellis2020privacy}.

Ichikawa \emph{et al.} \cite{ichikawa2017tamper} utilised an older Hyperledger Fabric version without private data collection, lacking Idemix suite support, compromising end-user privacy. Updating a newer Hyperledger version for private data collection would require a complete architectural redesign. Liang \emph{et al.} \cite{liang2017integrating} simulated a healthcare scenario with various entities, including users, healthcare providers, and insurance companies. However, newer Hyperledger versions introduced challenges that require a re-evaluation of their system. MeDShare \cite{xia2017medshare} discusses blockchain fundamentals more than specific solutions without a clear choice of blockchain framework.

A novel EHR management method combining permissionless blockchain, cloud storage, and medical IoT data is proposed in \cite{dwivedi2019decentralized}. It leverages lightweight symmetric and asymmetric encryption for anonymity and authorisation. However, its performance efficiency and GDPR compliance still need to be explored.

\subsubsection{Other implementations}
Sharma, Chen, and Sheth \cite{sharma2018toward} explored kHealth, a cloud-based system for managing health data from IoT devices. This system aims to develop personalised health predictive models, employing homomorphic encryption and differential privacy for robust privacy preservation. However, scalability optimisations can compromise these privacy measures.

Dubovitskaya \emph{et al.} \cite{dubovitskaya2015cloud} introduced a privacy-preserving e-Health cloud system, encrypting medical data using public-key cryptography for both local and cloud-stored databases. Patient-specified policies control access. However, the potential misconduct by cloud providers, such as IP address-based inference attacks, threatens user anonymity.

Casino \emph{et al.} \cite{casino2019systematic} examined how blockchain could revolutionise various healthcare applications, including EHR management, drug counterfeit prevention, and patient-centric medical research.

Ming and Zhang \cite{ming2018efficient} proposed an efficient Privacy-Preserving Access Control (PPAC) scheme for EHR in cloud-based systems. It combines the cuckoo filter with an Attribute-Based Signcryption (ABSC) mechanism, ensuring anonymity and computational efficiency. Despite comprehensive privacy guarantees, GDPR compliance remains unassessed.

Roehrs \emph{et al.} \cite{roehrs2017omniphr} distributed Personal Health Record (PHR) information into data blocks. Although appearing centralised, it is decentralised among participants. Their protocol, openPHR, is extensible and can be practically adopted by organisations. However, security and privacy concerns persist, and unlike EHR, which healthcare institutions control, PHRs are patient-controlled.

\section{IPFS use cases}\label{ipfs_usecases}
IPFS offers a decentralised P2P file system without a centralised server, likened to Torrent networks for its censorship resistance \cite{henningsen2020mapping}. Benet \cite{benet2014ipfs} describes IPFS as a web-like structure using content-address hyperlinks, integrating BitTorrent swarm object exchanges within a Git repository.

IPFS fragments files into blocks, utilising a Merkle DAG and a distributed hashtable. Unlike traditional blockchain, where transactions are sequentially stored, DAG makes each transaction a block, speeding up consensus. Lerner \cite{lerner2015dagcoin} highlighted that DAG transactions include their proof of work and advocated using a fast cache for recent transactions.

\subsection{Architecture}
Chen et al \cite{chen2017improved} 
defined four IPFS layers: storage (Layer 4), routing (Layer 3), virtual chain (Layer 2), and blockchain (Layer 1). The blockchain layer can either build a new blockchain or use Bitcoin's blockchain. Blockstack \cite{ali2017blockstack}, using Gaia distributed database \cite{sood2022decentralised}, stores data in web browsers rather than centralised servers, enhancing privacy. Stacks 2.1, built atop Bitcoin's blockchain, enables smart contracts and decentralised applications \cite{ali2020stacks}.

The virtual chain layer processes and verifies transactions, signing them with private and public keys. Transactions typically bind a node's IP address to its account and declare associated files. Files, either long-term immutable or occasionally mutable, are broken into blocks for exchange via the BitSwap protocol. BitSwap uses want-lists for block requests, promoting bartering between nodes. The routing layer maps account routing addresses to files or blocks, while the storage layer holds mutable and immutable data.

Chen et al \cite{chen2017improved} improved IPFS by introducing a zig-zag file storage structure, providing a triple replication scheme for frequently used (hot) data and an erasure codes storage scheme for infrequently used (cold) data. This approach differentiates between hot data, stored near computation for quick access, and cold data, suitable for cloud storage.

%The Blockstack framework is currently built on the Bitcoin blockchain, but can be moved onto another platform. 

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/chennew.png}
%\caption{IPFS Architecture %\cite{chen2017improved}}
%\label{chen}
%\end{center}
%\end{figure*}

\subsection{IoT Integration}

In the realm of IoT integration, Muralidharan et al. \cite{muralidharan2019interplanetary} have made significant strides by implementing an IoT network utilising the IPFS. This system uniquely addresses nodes and data through cryptographic hashes. It employs Distributed Hash Tables (DHTs) for routing and facilitating the efficient location and dissemination of data among peers. These DHTs also store data, potentially reducing latency in data access. The network's infrastructure remains current through a Merkle DAG and Git versioning. To bolster security, IPFS incorporates secure file sharing and encrypted communication methods.

Furthering this innovation, Nizamuddin et al. \cite{nizamuddin2019decentralized} have developed an IPFS framework integrated with Ethereum. Their work, including Solidity smart contracts, is documented on GitHub \cite{gitNizamuddin} and has undergone testing in Remix, an Ethereum Integrated Development Environment. This environment supports the development of smart contracts \cite{remix2021}. Their approach defines two primary roles: Developers (D) and Approvers (A), identified by Ethereum addresses. The creator initiates a smart contract for each document, with Developers responsible for uploading the document to the IPFS system. Notably, a two-thirds majority of new Developers/Approvers must receive approval from existing Approvers to be accepted.

\subsection{Performance}

The performance of IPFS was methodically measured by Henningsen et al. \cite{henningsen2020mapping} using a Kademlia-based DHT. Their study observed an average of 44,474 nodes, 52.19\% behind a Network Address Translation (NAT) system. They found the infrastructure robust, particularly in its resistance to Sybil attacks. However, they also noted performance weaknesses and concerns regarding the privacy of queries.

Naz et al. \cite{naz2019secure} have implemented a data-sharing model involving various entities:

- \textbf{Owner}: The entity sharing data, such as a government body.
- \textbf{Customer}: An entity downloading files from an IPFS server using reconstructed hashes.
- \textbf{Worker}: Assists in decrypting content for customers, authenticates new customers, and queries smart contracts regarding customer data requests.
- \textbf{Arbitrator}: Resolves disputes between content buyers and sellers.

In Naz's model \cite{naz2019secure}, an Owner generates metadata for a file to be shared, including filename, type, size, and description. This data, along with the complete file, is added to IPFS. Upon addition, the Owner receives back data hashes and contacts trusted worker nodes. These nodes, with key pairs stored in smart contracts, are tasked with decrypting content. The file hashes are divided into $k$ shares using the Shamir Secret Share (SSS) method, encrypted with $n$ random keys, and stored alongside security information on a blockchain. The encryption of these hashes is crucial to prevent adversaries from reconstructing the file. Valid customers, having paid for access, can then reassemble the files. These shares are encrypted in a smart contract and are accessible only to verified workers identified by their public key.

Ali et al. \cite{ali2017iot} employed a side-chain method for maintaining network privacy, where a validator node operates the side chain. Each IoT device in the network encrypts data using its public and private keys for the validator, who then adds this data to a side chain. A smart contract facilitates communication between the device and the validator, storing both the public key and IPFS hash, device data, and requesters' public key and access rights.

Kumar et al. \cite{kumar2019implementation} explored implementing IPFS networks to diminish the size of blockchain transactions and facilitate content-addressed access. Here, miners store transactions in the IPFS distributed storage and store the corresponding IPFS hash in a blockchain block.

\subsection{Applications}

Sun et al. \cite{sun2020blockchain} integrated ciphertext policy attribute-based encryption (CP-ABE) with IPFS to store and share electronic medical records securely. CP-ABE regulates access to encrypted files, while IPFS distributes the storage of these files. Their system comprises a Blockchain, IPFS, a medical system, and a data user (DU). Initially, a patient (Bob) receives a public-private key pair based on his attributes. During a hospital visit, Doctor Alice diagnoses Bob and encrypts this diagnosis with Bob's public key before uploading it to IPFS. Alice then encrypts the IPFS hash address with a random number, hashes the medical records and their index with SHA-256, and stores this data on the blockchain. Bob can access his records by verifying the hash address and downloading.


%A scenario for this is defined in Figure \ref{ransom}.

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/arg.png}
%\caption{Agricultural products tracking  %\cite{taborda2020decentralized}}
%\label{arg}
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/book.png}
%\caption{Book tracking system  %\cite{nizamuddin2018ipfs}}
%\label{book}
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/book2.png}
%\caption{Smart contract tracking system  %\cite{nizamuddin2018ipfs}}
%\label{book2}
%\end{center}
%\end{figure*}


%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/pi.png}
%\caption{Record keeping system on IPFS   \cite{vishwavidyapeetham2018blockchain}}
%\label{pi}
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.8\linewidth]{figures/bot.png}
%\caption{Hydras and IPFS: a decentralised playground for malware   %\cite{patsakis2019hydras}}
%\label{bot}
%\end{center}
%\end{figure*}




%\begin{figure*}
%\begin{center}
%\includegraphics[width=0.95\linewidth]{figures/ransom.png}
%\caption{Ransomware on IPFS %\cite{karapapas2020ransomware}}
%\label{ransom}
%\end{center}
%\end{figure*}









==> 03_ebsi.tex <==
\section{Overview of European Electronic Identity Systems}
\label{eu_eid}

The concept of identity, and by extension, electronic identity (e-ID), differs markedly across nations. Globally, notable e-ID implementations include the ICAO electronic passport system \cite{pasupathinathan2008line}, prevalent in most countries, and India's Aadhaar system \cite{khera2017impact}. Each country's political and cultural context influences trust in these systems. Interestingly, some nations lack a national identity scheme. For instance, the UK abandoned its national ID scheme, influenced partly by a blog post \cite{GOV.UK2011, Saunders2006}. 

\subsection{European Union's Approach to Electronic Identity}
\subsubsection{eIDAS Framework}
\label{subsubsec:eidas}
The European Commission's DG Connect initiated the eIDAS (electronic Identification, Authentication and trust Services) regulation, encompassing e-identification and trust services \cite{eidasreg}. This initiative is technically bolstered by ETSI and CEN, focusing on standard development. Implementing Decisions and Regulations specifically target e-identification \cite{eidasregia-ID-4} and trust services \cite{eidasregia-TS-4}, with additional rules covering e-signature products and Trusted Lists.

Delos et al. \cite{seletal2015eidas} detail how EU member states can independently manage their trust ecosystems. The FutureTrust project \cite{DBLP:conf/openidentity/HuhnleinFSPSHWN16} explored trust foundations, providing open-source tools for this purpose. Member states retain sovereignty in organising citizen identity, typically offering electronic authentication mechanisms like userid/password schemes, smart cards, and mobile applications.

A member state may notify the EU Commission of its identity management systems, leading to mutual recognition across the EU. Minimum identity attributes for natural and legal persons are established \cite{eidasregia-ID-2}. Trust Service Providers (TSPs), including Qualified Trust Service Providers (QTSPs), are monitored by national supervisory bodies. These bodies rely on Conformity Assessment Bodies (CABs), usually private firms, for TSP and QTSP evaluation.

CABs must be accredited by a National Accreditation Body (NAB) and publicly declare their conformity assessment scheme. The European Cooperation for Accreditation (EA) endorses an eIDAS accreditation scheme based on ISO/IEC 17065 \cite{ISO17065:2012} and ETSI EN 319 403 \cite{etsien319403}, as outlined in EA Resolution EA 2014 (34) 22 \cite{EA-resolution-2014-34-22}.

eIDAS Article 3 \cite{tsakalakis2017identity} establishes terminology and definitions for electronic signatures, categorising trust services into basic, advanced, and qualified levels. The EU Commission provides a legal, functional, and technical framework for evaluating and validating identity and trust services, including the publication of signed metadata and the List of Trusted Lists (LOTL).

\subsubsection{European Digital Identity Wallet}
The 2021 proposal \cite{EuropeanCommission2021a} recommended updates to eIDAS, mandating EU states to provide a European Digital Identity Wallet (EDIW). This initiative introduces four new Trust Services \cite{EuropeanCommission2021a, Thales2022}, enhancing support for distributed ledger technologies and electronic signature applications.

The pilot phase for EDIWs starts in 2023, aiming for EU-wide availability by 2024. These wallets are expected to be GDPR-compliant and integrate with the eIDAS framework. Thales's survey \cite{Thales} reveals varying perceptions and concerns among EU citizens regarding these wallets' privacy, security, and convenience.

\section{European Blockchain Partnership}
\label{eu_blockchain_part}
In 2018, the European Blockchain Partnership (EBP) was formed by 27 EU states, Norway, Liechtenstein, and later Ukraine \cite{queiruga2022self, EBP}. This partnership led to the European Blockchain Services Infrastructure (EBSI), targeting use cases like Self-Sovereign Identity and Diploma awards \cite{vasileedis}, Document Traceability, and Trust Data Sharing. The EBSI uses a public permissioned blockchain, with digital credentials stored in citizen-controlled wallets \cite{grech2021blockchain}. Baldacci et al. \cite{baldacci2021advancing} outline EBSI's core principles, including decentralisation, scalability, open specifications, sustainability, and interoperability.

In 2020, initiatives like DIZME, Findy, Lissi, and MeineSichereID collaborated within the Trust over IP Foundation \cite{EBSI2020}, aiming to create a unified European SSI Network. The European Commission has developed various blockchain strategies \cite{fulli2021policy}, including crypto-asset regulation \cite{sandner2022crypto} and market infrastructure development based on distributed ledger technology \cite{priem2022european}. These efforts are integral to the EBP and its investment in EBSI \cite{EBSI}.

\subsection{EBSI and Its Applications}
\subsubsection{The EBSI Project}
Turkanovic et al. \cite{turkanovic2020signing} describe EBSI's integration with EU public services, running on Hyperledger Besu \cite{dalla2021your} and Fabric clients. EBSI's ledger protocol allows for a pluggable design, adaptable to different client needs \cite{EBSI}. The infrastructure supports public reading access, with writing permissions limited to trusted entities. Figure \ref{fig:cocco} outlines the SSI model EBSI uses.

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/futureinternet-14-00140-g001.png}
\captionsetup{justification=centering}
\caption{SSI model for EBSI \cite{cocco2022system}}
\label{fig:cocco}
\end{center}
\end{figure*}


EBSI's use cases encompass identity verification, academic awarding, social security checks, and document traceability. The European Self-Sovereign Identity Framework (ESSIF) at EBSI's core is GDPR and e-IDAS compliant, enabling secure and legal identity management for EU citizens.

Bittins et al. \cite{bittins2021healthcare} discuss EBSI's potential for secure healthcare data sharing across the EU, leveraging blockchain technology for data provenance and integrating SSI.

\subsection{EBSI Compliance and Security}
EBSI aligns with several regulations, including the NIS Directive \cite{directive2016directive}, the eIDAS Regulation, and GDPR. Its security framework mandates appropriate measures for safeguarding the infrastructure and the applications built upon it. These measures are essential for maintaining the reliability and integrity of the EBSI network and its services.  A selection of key security measures of the framework is listed in Table \ref{table:1}.

\begin{table*}[]
\begin{center}
\caption{A selection of EBSI V2 Security Measures}
\begin{tabular}{p{4cm} | p{7cm}}
Security Measure ID & Security Measure Description \\
\hline
EBSI\_V2\_SMID\_001             & End user identification/authentication based on EU Login and EBSI wallet (covering users)\\
EBSI\_V2\_SMID\_002 & DevOps users identification/authentication based on remote SSH login\\
EBSI\_V2\_SMID\_003 & Application components identification/authentication based on JSON Web Token (JWT) and component key pairs (covering components and enterprises)\\
EBSI\_V2\_SMID\_004 & EBSI API acts as an access mechanism for blockchain and distributed storage services\\
EBSI\_V2\_SMID\_005 & Registry of trusted dapps in a smart contract\\
EBSI\_V2\_SMID\_006 & Registry of trusted issuers (governments and universities) in a smart contract\\
EBSI\_V2\_SMID\_007 & Registry of trusted accreditation organisations in a smart contract\\
EBSI\_V2\_SMID\_007 & Registry of trusted registration authorities in a smart contract\\
EBSI\_V2\_SMID\_009 & Registry of trusted schemes in a smart contract\\
EBSI\_V2\_SMID\_010 & Protection of all smart contracts by an ABAC[7] security policy and a multi-sig smart contract\\
EBSI\_V2\_SMID\_011 & All EBSI front-end components have a TLS[8] certificate\\
EBSI\_V2\_SMID\_012 & All EBSI front-end components are protected by a proxy server\\
EBSI\_V2\_SMID\_013 & All EBSI components are protected by a firewall\\
EBSI\_V2\_SMID\_014 & All EBSI  components run on a hardened Operating System\\
EBSI\_V2\_SMID\_015 & For those EBSI  components that are cloud-based, the cloud provider's security \\
\end{tabular}
\label{table:1}
\end{center}
\end{table*}



























==> 04_glass.tex <==
\section{The GLASS Project: A Study of Distributed Ledger Technology}\label{sec:Background}

The GLASS project adopts a distributed domain approach as shown in Figure~\ref{jain1}. The project is based on Hyperledger Fabric, a platform used for building blockchain applications. In this instance, three sovereign nations collaborate on a single channel to enhance their governance infrastructure. Each nation comprises two departments responsible for the endorsement, validation, and recording of citizen data. These departments sign identity documents using private keys and verify them with public keys on the EBSI ledger.
  
\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/distributed_example.png}
\caption{An overview of a distributed data-sharing platform  based on permissioned blockchain.}
\label{jain1}
\end{center}
\end{figure*}

\subsection{Decentralised Distributed Ledger and Chaincode}
Blockchain technology in the GLASS project is characterised as decentralised, resistant to tampering, and distributed across peer-to-peer networks~\cite{Papadopoulos2020}. Coupled with smart contracts, it provides a structure for developing access control mechanisms vital for secure identification, authentication, and user authorisation. The immutable ledger of the blockchain safeguards against integrity issues. Smart contracts enable the implementation of programmable policies for user authentication and authorisation in a distributed setting~\cite{MarkoHolbl}.

In Hyperledger Fabric, a permissioned blockchain, the chaincode links with the ledger and forms the core of the blockchain system~\cite{chaincode}. The chaincode runs on peers within an organisation, managing the creation, querying, and updating of transactions on the shared ledger. It is instrumental in formulating asset definitions for business contracts and managing decentralised applications.

\subsection{Interplanetary File System}
The InterPlanetary File System (IPFS) is a significant element in the GLASS project~\cite{benet2014ipfs, ipfs}. This protocol allows for the distributed storage and transfer of digital content using a peer-to-peer model and content-based addressing. Similar to BitTorrent, IPFS's distributed nature facilitates file sharing across a network. IPFS can create a permanent and distributed web system, either public or private. It replaces the traditional URL system with cryptographic hashes as addresses. In the IPFS network, data is distributed without a central point, and peers become distributors of content once downloaded. Digital assets like folders, images, and data stores are segmented and stored distributedly, each piece content-addressed using a Content Identifier (CID).

\subsection{Content Identifier and Distributed Hash Table}
A CID in IPFS serves as a unique marker for resources, focusing on content rather than its location, unlike URLs~\cite{Multiformats2020}. CIDs maintain a fixed length and are cryptographic hashes of the content. Any change in data results in a different CID. The Distributed Hash Table (DHT) acts as a decentralised key-value storage system, serving as a distributed database for storing and retrieving information based on node keys~\cite{benet2014ipfs}. Its main function is to link a CID to the content's location in IPFS.

\subsection{Distributed Infrastructure of Trust and Triplets Design}
The GLASS project's trust infrastructure is based around domains specific to each country, illustrated in Figure~\ref{fig:trip02}. This includes mapping digital signers specific to each country and their rights. Departments like the Department of Justice in the [DE] country domain have signing keys, which are stored in Hyperledger along with their public keys, identity (ID), and claim rights.

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/trip02.png}
\caption{Overview of the trust infrastructure.}
\label{fig:trip02}
\end{center}
\end{figure*}

The triplets design in Hyperledger Fabric is the primary metadata, enabling decryption of data distributed on IPFS. Figure~\ref{fig:trip01} shows each citizen's credential file encrypted with a unique key using the AES GCM method. The encrypted key, along with the file's CID and location (URI), is stored. The URI may link to an IPFS store or a URL.

\begin{figure*}
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/trip01.png}
\caption{Overview of triplets.}
\label{fig:trip01}
\end{center}
\end{figure*}

The trust within each domain is supported by storing the public key of credential signers (Figure \ref{fig:trust03}). These signers are trusted for specific credential types as outlined in the trust policy. The signers' public key structure corresponds to that shown in Figure \ref{fig:trip02}. The architecture ensures that the URI of the encrypted credential is stored, but the file contents are inaccessible, retrievable only by the citizen's private key.

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/trust03.png}
\caption{Trust infrastructure within ledger.}
\label{fig:trust03}
\end{center}
\end{figure*}

\subsection{Resource Distribution and Integration}
The GLASS project employs the InterPlanetary File System as its primary protocol for resource distribution. The current prototype encrypts all resources distributed on IPFS, using a private instance of IPFS for enhanced security. This private network operates like the public version, but only nodes with a shared private key can access it, preventing inadvertent exposure of sensitive information.

In integrating Hyperledger Fabric with IPFS, the GLASS project uses both CID and URI to store the same content on IPFS. The separate field property of URI allows future content distribution through various mechanisms, such as Dropbox and SharePoint. In these cases, the CID remains unchanged, but the URI varies based on the resource location. This design allows for the encryption key to be hosted in an external domain, adding flexibility and security to the system.

==> 05_GLASS_over_EBSI.tex <==
\section{Analysis of GLASS e-Governance and EBSI Infrastructure Integration}
\label{glass_ebsi}

This section explains the architecture reference model’s fundamental components and potential applications, focusing on integrating the GLASS data-sharing model with the EBSI infrastructure. A generic model and a use-case scenario model are employed for this assessment. The high-level design of the reference model is depicted in Figure \ref{fig:glassover}. An overview of GLASS and EBSI components and their essential services is provided prior to delving into the architecture specifics.


\begin{figure*}[h]
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/GLASS_EBSI_1.png}
\captionsetup{justification=centering}
\caption{GLASS and EBSI layers}
\label{fig:glassover}
\end{center}
\end{figure*}

\subsection{EBSI}
\subsubsection{Business Application}
Integrating GLASS-related business applications within the EBSI framework primarily aims to facilitate the merging of public and private sector applications. This integration occurs either through core service APIs or by hosting a node within the network. The EBSI business interface permits applications to utilise the EBSI-exposed API interfaces, enabling transactions with smart contracts in the EBSI ledger.

\subsubsection{Use Cases}
EBSI use cases to demonstrate its capability to provide public services across international boundaries. These cases are designed to streamline administrative processes and validate the integrity of digital information across various sectors. This approach enhances efficiency and public trust. The initial use cases in EBSI Version 1 include notarisation of documents, diploma management, European Self-Sovereign Identity, and trusted data exchange. Additional use cases, such as SME finance, asylum, and the European Social Security Platform, were subsequently introduced.

\subsubsection{Core Services}
The core services layer includes functionalities applicable to any use case. It provides interfaces for various EBSI services, encompassing both on-chain and off-chain components, and contains application enablers. These microservices are categorised into five distinct groups, offering tools like the Integration API, trusted registries, API security management, and the wallet library. Additionally, digital identity-related features are accessible through this layer.

\subsubsection{Chain and Storage}
This layer comprises supported distributed ledger and storage protocols. The EBSI V2 Ledger API facilitates user interaction with Hyperledger Besu (Read and Write) and Fabric ledgers (Read Only) \cite{li2020survey}. Smart contracts within this layer manage and execute trusted transactions for recording on the blockchain.

\subsubsection{EBSI Infrastructure}
The EBSI infrastructure layer provides general capabilities and connectivity to blockchain networks, including network, compute, and deployment capabilities. It encompasses all components necessary for establishing an EBSI node. The ledger validates, approves, and stores transactions on the blockchain. Presently, 25 nodes hosted by participating member states form this decentralised network.

\subsection{GLASS}
The GLASS architecture, reliant on a trust infrastructure spanning country-wide domains, facilitates distributed trust infrastructure amongst EU member states. Parallel to EBSI, GLASS provides an e-governance framework for use by EU member states, leveraging distributed ledger technologies for efficient, transparent, and user-friendly public service solutions.

\subsubsection{Business Application}
This layer aims to bridge connections between entities legally permitted to utilise GLASS services. It includes a user’s wallet, an essential management tool providing a graphical interface for managing digital keys. These keys assist in signing transactions, credentials, and documents, enabling secure interactions and relationships with third parties.

\subsubsection{Use Cases}
GLASS’s primary use cases involve relocation to another Member State, short-term visits to other countries, and securing employment abroad \cite{glassusecase}.

\subsubsection{Core Services}
The core services of GLASS establish connections between the GLASS portal, Hyperledger Fabric ledger, and a private IPFS network instance, forming a trusted e-governance data-sharing model. These services comprise various identity trust capabilities and APIs, enabling blockchain-based services to achieve high identity assurance and trust standards. Services include credential signing and sharing, ledger transactions, encryption, and APIs for issuing verifiable credentials linked to electronic identification (eID).

\subsubsection{GLASS Portal}
The GLASS portal integrates distributed ledger technologies with a private IPFS network instance for recording and storing encrypted verified credentials on a Hyperledger fabric ledger with restricted access. It facilitates sharing encrypted resources over a private IPFS cluster, creating a Content Identifier (CID) for the resource. The portal also interacts with Hyperledger Fabric to record the CID, URI, and encryption keys. Upon completing these processes, users receive a CID and URI for their encrypted resource, enabling future retrieval.

\subsubsection{Chain and Storage}
GLASS employs IPFS for storage, integrating it with Hyperledger Fabric. The system’s architecture utilises URI, CID, and a Protected Encryption Key for security, which can store these elements in a secure Hyperledger Fabric record within the EBSI architecture. Hyperledger Fabric’s internal ‘chaincode’ facilitates transactions and ledger updates. A specific GLASS-ipfs chaincode in Hyperledger Fabric allows for the creation and reading of Glass resource keys.

\subsubsection{GLASS Ledger}
The GLASS ledger, a permissioned blockchain on Hyperledger Fabric, stores encrypted and disseminated resource triplets (CID, Key, URI) on IPFS. These triplets are stored in hashed form for security. Two types of data collection are utilised: one public (readable by both participating organisations) and one private (accessible only by org1.org). This setup aligns with the proposed Triplet concept.

\subsection{GLASS over EBSI Model}
The GLASS over EBSI model integrates numerous identity trust components for high assurance in blockchain-based services. This model can utilise EBSI services, incorporating eSignature and eID properties for EU cross-border identification. It ensures robust linkages between a user’s digital and physical identities by encrypting and storing credentials on IPFS, verifiable by all EU state members.

In this model, GLASS provides wallet functionality for citizens and organisations, enabling user identification and association with DIDs in the EBSI ledger. The model is illustrated in Figure \ref{fig:overeb}, depicting identifiers for citizens and organisations (legal and natural persons).

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/GLASS_EBSI_4.png}
\captionsetup{justification=centering}
\caption{GLASS over EBSI model}
\label{fig:overeb}
\end{center}
\end{figure*}

Client wallets use the EBSI wallet API to generate key pairs, initiating the onboarding process for recording information in the EBSI ledger. Authorised issuers and individuals are registered in the EBSI ledger via dedicated APIs, facilitating verification processes within the ecosystem.

The model (Figure \ref{fig:overeb}) outlines various processes:

\begin{itemize}
    \item Students can request and present verifiable university credentials to prospective employers in other countries.
    \item Universities issue encrypted certificates, with GLASS portals facilitating secure resource distribution via private IPFS networks.
    \item The use of AES-256 CBC for encryption and automatic distribution of resources on IPFS is detailed, highlighting security measures.
    \item The GLASS portal records metadata triplets (CID, encryption key, URI) in Hyperledger Fabric data collections for auditing and retrieval.
    \item Verification processes involve students presenting credentials to employers, with verifiers querying the EBSI ledger to confirm issuer DIDs.
\end{itemize}

The GLASS and EBSI integration demonstrates a robust cross-border e-governance and data-sharing framework. This underscores the importance of secure, transparent, and efficient digital identity management in the European Union.

==> 06_conclusion.tex <==




\section{Conclusion}\label{sec:Conclusion and future work}

At its core, enhanced e-governance could increase government services’ efficiency, quality, and effectiveness. However, many political narratives can stall its development, including the digital divide, anti-corruption, the loss of privacy, social change, and the increasing control from government agencies \cite{draheim2020narratives}.  

GLASS \cite{chrysoulas2021glass} focuses on developing an e-governance framework that the European Union’s member states could adopt, while EBSI focuses on providing trusted identity data. Key features of EBSI are the provision of GDPR compliance and eIDAS 2 signatures. The two infrastructures could thus provide an integrated approach to enhanced e-governance services across the EU and support EU citizens' freedom of movement in the future.









